Shrinkage under Random Projections, and Cubic Formula Lower Bounds for $\mathsf{AC}^0$

$\newcommand{\ACz}{\mathbf{AC}^0}$ H\r{a}stad showed that any De Morgan formula (composed of AND, OR and NOT gates) shrinks by a factor of $\tilde{O}(p^{2})$ under a random restriction that leaves each variable alive independently with probability $p$ [SICOMP, 1998]. Using this result, he gave an $\widetilde{\Omega}(n^{3})$ formula size lower bound for the Andreev function, which, up to lower order improvements, remains the state-of-the-art lower bound for any explicit function. In this paper, we extend the shrinkage result of H\r{a}stad to hold under a far wider family of random restrictions and their generalization -- random projections. Based on our shrinkage results, we obtain an $\widetilde{\Omega}(n^{3})$ formula size lower bound for an explicit function computable in $\ACz$. This improves upon the best known formula size lower bounds for $\ACz$, that were only quadratic prior to our work. In addition, we prove that the KRW conjecture [Karchmer et al., Computational Complexity 5(3/4), 1995] holds for inner functions for which the unweighted quantum adversary bound is tight. In particular, this holds for inner functions with a tight Khrapchenko bound. Our random projections are tailor-made to the function's structure so that the function maintains structure even under projection -- using such projections is necessary, as standard random restrictions simplify $\ACz$ circuits. In contrast, we show that any De Morgan formula shrinks by a quadratic factor under our random projections, allowing us to prove the cubic lower bound. Our proof techniques build on H\r{a}stad's proof for the simpler case of balanced formulas. This allows for a significantly simpler proof at the cost of slightly worse parameters. As such, when specialized to the case of $p$-random restrictions, our proof can be used as an exposition of H\r{a}stad's result.

==> tocspecial.tex <==
%% tocspecial.tex 2020-09-01  Version 0.22  ToC style file
%------------------------------------------------------------------
% Filename: tocspecial.cls
% 
% This documentclass is intended for typesetting articles for the
% 
% Theory of Computing.
% 
% See http://theoryofcomputing.org for further details.
%
% Version 0.1 Initial combination of banners from previous style files.
% Version 0.2 Addition of CCC banners. Clean up.
% Version 0.21 Addition of more CCC banners, up to 2023
% Version 0.22 Rename \boolean --> \aboolean to avoid clash with ifthen.
% ------------------------------------------------------------------
%
%% Special issue banners:

%% explanation: BC = 2012 BD = 2013 ... CA = 2020 CB = 2021 ...

\newcommand{\motwani}{Special issue in honor of Rajeev Motwani}
\newcommand{\aboolean}{Special issue: Analysis of Boolean Functions}
\newcommand{\approxrandomBC}{Special issue: APPROX-RANDOM 2012}
\newcommand{\approxrandomBD}{Special issue: APPROX-RANDOM 2013}
\newcommand{\approxrandomBE}{Special issue: APPROX-RANDOM 2014}
\newcommand{\approxrandomBF}{Special issue: APPROX-RANDOM 2015}
\newcommand{\approxrandomBG}{Special issue: APPROX-RANDOM 2016}
\newcommand{\randomBI}{Special issue: RANDOM 2018}
\newcommand{\approxrandomBJ}{Special issue: APPROX-RANDOM 2019}
\newcommand{\cccBF}{Special issue: CCC 2015}
\newcommand{\cccBG}{Special issue: CCC 2016}
\newcommand{\cccBH}{Special issue: CCC 2017}
\newcommand{\cccBI}{Special issue: CCC 2018}
\newcommand{\cccBJ}{Special issue: CCC 2019}
\newcommand{\cccCA}{Special issue: CCC 2020}
\newcommand{\cccCB}{Special issue: CCC 2021}
\newcommand{\cccCC}{Special issue: CCC 2022}
\newcommand{\cccCD}{Special issue: CCC 2023}

